LAPRAN: A Scalable Laplacian Pyramid Reconstructive Adversarial Network for Flexible Compressive Sensing Reconstruction

This paper addresses the single-image compressive sensing (CS) and reconstruction problem. We propose a scalable Laplacian pyramid reconstructive adversarial network (LAPRAN) that enables high-fidelity, flexible and fast CS images reconstruction. LAPRAN progressively reconstructs an image following the concept of Laplacian pyramid through multiple stages of reconstructive adversarial networks (RANs). At each pyramid level, CS measurements are fused with a contextual latent vector to generate a high-frequency image residual. Consequently, LAPRAN can produce hierarchies of reconstructed images and each with an incremental resolution and improved quality. The scalable pyramid structure of LAPRAN enables high-fidelity CS reconstruction with a flexible resolution that is adaptive to a wide range of compression ratios (CRs), which is infeasible with existing methods. Experimental results on multiple public datasets show that LAPRAN offers an average 7.47dB and 5.98dB PSNR, and an average 57.93% and 33.20% SSIM improvement compared to model-based and data-driven baselines, respectively.

==> Training.tex <==
\subsection{Training G}
	 
		
		The content loss also helps to overcome the mode collapse problem. In a batch, samples come from multi-modes and the content loss directly encourages the diversity in output.
		
		We also try to add a data-consistency loss \cite{CycleGAN2017Zhu,Tran2017cyclic} to ensure the generated image can be projected onto the original compressed manifold. However, we find the recovery accuracy is not improved which proves the generated images approximates the original image distribution quite well. So we abandon the data-consistency loss in the proposed model. By removing this layer, the reconstruction time cost is also decreased accordingly. 
		
		During the back-propagation, only the current stage is updated and all the prior stages remain unchanged. When we back-propagate to the prior stages, the recovery quality of the prior stages degrade.
		
		We find the performance is not sensitive to the number of convolution layers in the latter sub-networks. Also, to facilitate the weight transfer, we use identical convolutional structure in each sub-network. 
		
	
	
